ChartAdapter: Large Vision-Language Model for Chart Summarization

Chart summarization, which focuses on extracting key information from charts and interpreting it in natural language, is crucial for generating and delivering insights through effective and accessible data analysis. Traditional methods for chart understanding and summarization often rely on multi-stage pipelines, which may produce suboptimal semantic alignment between visual and textual information. In comparison, recently developed LLM-based methods are more dependent on the capability of foundation images or languages, while ignoring the characteristics of chart data and its relevant challenges. To address these limitations, we propose ChartAdapter, a novel lightweight transformer module designed to bridge the gap between charts and textual summaries. ChartAdapter employs learnable query vectors to extract implicit semantics from chart data and incorporates a cross-modal alignment projector to enhance vision-to-language generative learning. By integrating ChartAdapter with an LLM, we enable end-to-end training and efficient chart summarization. To further enhance the training, we introduce a three-stage hierarchical training procedure and develop a large-scale dataset specifically curated for chart summarization, comprising 190,618 samples. Experimental results on the standard Chart-to-Text testing set demonstrate that our approach significantly outperforms existing methods, including state-of-the-art models, in generating high-quality chart summaries. Ablation studies further validate the effectiveness of key components in ChartAdapter. This work highlights the potential of tailored LLM-based approaches to advance chart understanding and sets a strong foundation for future research in this area.

==> contents/charts_chart2text_stages.tex <==

\begin{figure*}
\centering
\subfigure[Template-based Approaches]{\label{fig:chart2text:a}
\includegraphics[width=0.45\linewidth]{images/chart2text_stage1.png}}
\hspace{0.01\linewidth}
\subfigure[Bi-model Approaches]{\label{fig:chart2text:b}
\includegraphics[width=0.45\linewidth]{images/chart2text_stage2.png}}
\vfill
\subfigure[LVLM-based Approaches]{\label{fig:chart2text:c}
\includegraphics[width=0.45\linewidth]{images/chart2text_stage3.png}}
\hspace{0.01\linewidth}
\subfigure[Our Approach]{\label{fig:chart2text:d}
\includegraphics[width=0.45\linewidth]{images/chart2text_stage4.png}}
\caption{\textbf{Overall Pipelines of Chart-to-text Summarization}. Subfigure (a-c) shows the existing pipelines of related works. (a) shows template-based approaches in the early stage, which generates fill-in descriptions based on the extracted data table. (b) shows recent LVLM-based approaches, which process the chart image via the Visual Component. (c) shows Bi-model approaches that adopt a frozen Visual Component to extract the data table as LLM's input. (d) demonstrates the pipeline of our design. }
\label{fig:chart2text}
\end{figure*}

==> contents/experiments/ablation_experiment.tex <==
% \subsection{Ablation Experiments}

% To fully verify our design, several ablation experiments are defined as follows, 

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=1\linewidth]{images/pre_merging.png}
% %     \caption{Pre-merging in Qwen2VL}
% %     \label{fig:pre_merging}
% % \end{figure}
% % \begin{figure}
% %     \centering
% %     \includegraphics[width=1\linewidth]{images/post_merging.png}
% %     \caption{post-merging in TinyChart}
% %     \label{fig:post_merging}
% % \end{figure}

% The ablation experiment of \textbf{different visual token merging} takes Qwen2VL-based implementation (fig \ref{fig:pre_merging}) as representatives of pre-merging and TinyChart-based implementation (fig \ref{fig:post_merging}) as representatives of post-merging. The pre-merging strategy merges subsequence similar chart patches according to the raw data, while the post-merging coalesces semantically similar representations ignoring the patch structures. 

% The ablation experiment of \textbf{Multi-stage Training Strategy} was presented in the following comparative groups, 


% \begin{enumerate}[label=\textit{(\alph*)}]
%     \item \textbf{Stage 1: CLIP Style Pretraining} can be verified by \textit{\textbf{Ours-Qwen2VL / TinyChart}} compared to \textit{\textbf{Ours-Qwen2VL / TinyChart w/o clip}} and \textit{\textbf{Ours-TinyChart scratch}} compared to \textit{\textbf{Ours-TinyChart scratch + clip}}. 
    
%     \item \textbf{Stage 2: Text Component initialization} can be displayed by \textit{\textbf{Ours-Qwen2VL}} compared to \textit{\textbf{Ours-Qwen2VL single}}. 
%     \item \textbf{Stage 3: Joint training} can be reviewed by \textit{\textbf{Ours-Qwen2VL}} compared to \textit{\textbf{Ours-Qwen2VL LLM only}} and \textit{\textbf{Ours-Qwen2VL TeT only}}. The \textit{\textbf{Ours-Qwen2VL LLM only}} is similar to the bi-model solution where components were loaded from other pre-train tasks and were frozen and only updates the LLM backbones. 
% \end{enumerate}

Several ablation experiments are conducted to fully verify our ChartAdapter design and training strategy. An overview of each setting is revealed in Table.~\ref{Table:exp_control_groups_definition}. 

\input{contents/experiments/ablation_group_table}

To evaluate the effect of the contrastive learning stage, we implemented an ablation group with the same settings as the experimental group, except for the training strategy. In this group, the projector network of ChartAdapter is randomly initialized and directly starts from the cross-modal summarization learning stage. We labeled this group as \textit{\textbf{Ours-Qwen2VL w/o clip}}. 

To evaluate the effect of the cross-modal summarization learning stage, we implemented an ablation group without the contrastive learning stage. This group used the projector network trained by the contrastive learning stage to jointly optimize the ChartAdapter and the LLM backbone. We labeled this group as \textit{\textbf{Ours-Qwen2VL single}}. 

To evaluate the effect of the jointly training stage, we implemented two groups which either update the ChartAdapter or the LLM backbone with the latent textual embeddings separately during stage 2 and stage 3. We labeled these groups as \textit{\textbf{Ours-Qwen2VL TeT only}} and \textit{\textbf{Ours-Qwen2VL LLM only}}. Simultaneously, the \textit{\textbf{Ours-Qwen2VL LLM only}} group shares a similar training strategy with Bi-model approaches. 

% including 11% of program-of-thought and 40% of data-table-extraction
Additionally, we implemented our ChartAdapter design based on TinyChart~\cite{zhang2024tinychart}, which is a SOTA model in the Chart-to-text field, to evaluate the effect of our backbone model. TinyChart~\cite{zhang2024tinychart} has a bipartite token merging strategy in the alignment phase and was trained on extract tasks, unlike the mainly textual-based tasks in Qwen2VL. This group was directly jointly trained with the projector network inherited from the contrastive learning stage and was labeled as \textit{\textbf{ Ours-TinyChart}}. 

To further verify the effects of inheriting from pre-trained LVLMs, we implemented a \textit{\textbf{Ours-TinyChart scra}} group with the same setting as \textit{\textbf{Ours-TinyChart}}, except all parameters were trained from randomly initialized. Furthermore, we also implemented the \textit{\textbf{Ours-TinyChart scra + clip}} with pre-trained projector network and \textit{\textbf{Ours-TinyChart w/o clip}} with randomly initialed projector network for \textit{\textbf{Ours-TinyChart }}, to eval the effect of the contrastive learning stage in different convergence processes. 


==> contents/experiments/dataset.tex <==




==> contents/results/ablation_experiments.tex <==
\subsection{Results of Ablation Experiments}

\input{contents/results/table_ablation_exp}

Each part of our training pipeline collectively accelerates convergence speed and improves overall performance. Details of each group are shown in Table.~\ref{Table:model_ablation_experiment}. 


Firstly, the \textbf{Contrastive Learning Stage} is beneficial to the joint optimal convergence, especially in the initial phase. Results between \textit{\textbf{Ours-TinyChart}} and \textit{\textbf{Ours-TinyChart w/o clip}} showed a 38.34\% relevant raise in the BLEU-4 metric (from 8.82 to 12.29) as well as an average 15.93% relevant increase in Rough-related metrics. 
But the optimal performance in \textit{\textbf{Ours-Qwen2VL}} and \textit{\textbf{Ours-Qwen2VL w/o clip}} fluctuates around a non-significant 2\% range. This indicates the acceleration of training convergence, especially in the initial state of \textit{\textbf{Ours-TinyChart scra + clip}}. 


Secondly, the \textbf{Summarization Learning Stage} has a slight improvement to the optimal performance. The result shows a 3\% raise in BLEU-4 from 34.48 to 35.55 and an average 3.8\% increase in Rough-related metrics between \textit{\textbf{Ours-Qwen2VL}} and \textit{\textbf{Ours-Qwen2VL single}}. Considering the similar optimal performance in the contrastive learning stage, the summarization learning stage helps improve the chart summarization capability by optimizing the ChartAdapter for better initiation under the unified LVLM space. 

Thirdly, the \textbf{Joint Training Stage}, which jointly optimized the ChartAdapter and the LLM backbone, is essential for the chart summarization performance. Missing any of these parts can lead to a drastic performance degradation, with 28.83 of BLEU-4 score in \textit{\textbf{Ours-Qwen2VL TeT only}} and 8.63 of BLEU-4 score in \textit{\textbf{Ours-Qwen2VL LLM only}}. Weak capabilities in \textit{\textbf{Ours-Qwen2VL LLM only}} the untrained encoder structure parameters in the decoder structure of cross-modal interaction network and implicit semantic decoder network. These also illustrate the boundaries of the Bi-model approaches when using a mismatch pre-trained component. 

Additionally, our success greatly relies on the powerful pre-trained parameters that are inherited from the backbone LVLM. Even the current SOTA model Qwen2VL~\cite{Wang2024qwen2vl} outperforms in the Chart-to-text Summarization fields. Training from scratch reveals an awful performance when optimizing such a larger scale of untrained parameters. 

In conclusion, our work has achieved significant results in bridging the gap between charts and textual summaries. 

==> contents/results/main_experiment.tex <==
\subsection{Results of Our ChartAdapter Design}

In general, \textit{\textbf{Ours-Qwen2VL}} (BLEU-4: 35.55, Rouge-1: 41.49, Rouge-2: 15.57, Rough-L: 25.79) generates summaries with more accurate wordings, more fluent sentences, and more precise descriptions compared to existing methods, even to the SOTA model TinyChart with BLEU-4 scores 17.18. 
Our ChartAdapter design enhanced the Qwen2VL model with outperformed capabilities to an even larger version. 
Efficient improvements have been accomplished through our ChartAdapter implementation, with a slight scaling (parameter size from 2 billion to 3 billion) achieving significant improvement to the backbone even with a larger scale. 
Improvement contains a 17.87\% relevant improvement in BLEU-4 and an average relevant improvement of 13.21\% in Rough-related metrics, indicating a robust chart summarization ability. More details can be referred to Table.~\ref{Table:model_performance}. 


% \input{contents/results/table_contrastive_learning}

Moreover, Qwen2VL~\cite{Wang2024qwen2vl} is more suitable to be the backbone model than TinyChart~\cite{zhang2024tinychart}, a SOTA model of the Chart-to-text Generation field. The BLEU-4 metric decreased from 17.18 to 12.29 during the TinyChart-based implementation. However, the projector network had a better result in \textit{\textbf{Ours-TinyChart}} than \textit{\textbf{Ours-Qwen2VL}} in the contrastive learning stage. Both of them achieved high AUC scores, while other binary classification metrics show a less favorable performance (with an average gap of 25\% in accuracy, precision, recall, and f1-score.) in Qwen2VL-based implementation, because of its much larger vocab size. Details can be obtained in Table.~\ref{Table:clip_pretrain_performance}. Yet, the TinyChart-based implementation is still leading in this stage. 

% \input{contents/results/table_generated_description}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/generated_summary_with_chart.png}
    \caption{Generated Summarization Sample}
    \label{fig:sample_generation}
\end{figure}

Furthermore, the generated chart summaries explain \textit{\textbf{Ours-TinyChart}}’s unsatisfying result, examples are shown in Table.~\ref{Table:generated_outcomes}. The TinyChart-based implementation suffered from defectives inherited from its pre-training tasks. On one hand, outcomes involved type recognition errors that were misidentified as other tasks. On the other hand, non-textual structured forms in other tasks occasionally lead to repeat errors in punctuation and the tabular symbol. Besides, token merging in the alignment phase ignores the patch structure and heavily relies on the accurate representation of the chart encoder. 

Therefore, Qwen2VL~\cite{Wang2024qwen2vl} is a more suitable backbone for our ChartAdapter. 


==> contents/results/table_contrastive_learning.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{c c c c c}
    \toprule
        AUC & Accuracy & Precision & Recall & F1  \\ \midrule
         0.98 & 70.69 & 71.75 & 70.68 & 70.65  \\ \midrule
    \end{tabular}
    \caption{Performances of the fine-tuned cross-modal projector in ChartAdapter}
    \label{Table:clip_pretrain_performance}
\end{table}

==> contents/results/table_generated_description.tex <==

\begin{table}[ht]
    \centering
    \begin{tabular}{p{1.5cm}|p{6cm}}
    \toprule
        Type  & Textual Content \\ \midrule
        % \, & Input  & $<$image$>$$\backslash$nWrite a summary for this chart. \\ \midrule
        % \, & Label  & The new Republican-led Congress is drawing harsh reviews from the public – including most Republicans. Just 23\% of Americans say congressional Republicans are keeping the promises they made during last fall’s campaign, while 65\% say they are not. \\ \midrule
        Label  & The new Republican-led Congress is drawing harsh reviews from the public – including most Republicans. Just 23\% of Americans say ...... \\ \midrule
        % Ours-TinyChart-tec &  Task Type Error  & $\backslash$t$\backslash$t (color: The Republican, 2015, 2012, 2011, the following the 28. The Republican Party’s: The `` Vote: The public opinion poll: Vote: The Democratic Party (2012. \\ \midrule
        % Ours-TinyChart-tec & Repeat Error  & $\backslash$t$\backslash$t, this chart is !!!!!!!. \\ \midrule
        % ChartAdapter & Output Summary & The public continues to say that the new Congress has done less than expected than expected in its first six days of session, but the proportion saying this has done less than expected has declined from 52\% in early 2011, when the tea party first emerged, to 46\% in January of this year. ...... A smaller majority (35\%) says the deficit has been a lower priority than expected. And a small minority (5\%) say that the deficit has been completely neglected. \\ \midrule
        ChartAdapter & The public continues to say that the new Congress has done less than expected than expected in its first six days of session, but the proportion saying this has done less than expected has declined from 52\% in early 2011, when the tea party first emerged, to 46\% in January of this year. ...... \\ \midrule
        
    \end{tabular}
    \caption{Generated Summarization}
    \label{Table:generated_outcomes}
\end{table}


==> contents/results/table_generated_with_chart.tex <==
% \usepackage{graphicx}

% \begin{tabular}{|c|c|}
% \hline
% Generated Response & Chart \\
% \hline
% The public continues to say that the new Congress has done less than expected than expected in its first six days of session, but the proportion saying this has done less than expected has declined from 52\% in early 2011, when the tea party first emerged, to 46\% in January of this year. ...... & \includegraphics[width=0.5\textwidth]{images/4616} \\
% \hline
% \end{tabular}

% \begin{table}[ht]
%     \centering
%     \begin{tabular}{p{6cm}|p{1.2cm}}
%     \toprule
%         Generated Response & Chart \\ \midrule
        
%          & \includegraphics[width=1.2cm]{images/4616} \hline
        
%     \end{tabular}
%     \caption{Generated Summarization}
%     \label{Table:generated_outcomes}
% \end{table}


==> refe_old.tex <==
\begin{thebibliography}{00}
\bibitem{b1} Cui C, Ma Y, Cao X, et al. A survey on multimodal large language models for autonomous driving[C]//Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision. 2024: 958-979.
\bibitem{b2} Yao B Z, Yang X, Lin L, et al. I2t: Image parsing to text description[J]. Proceedings of the IEEE, 2010, 98(8): 1485-1508.
\bibitem{b3} Aker A, Gaizauskas R. Generating image descriptions using dependency relational patterns[C]//Proceedings of the 48th annual meeting of the association for computational linguistics. 2010: 1250-1258.
\bibitem{b4} Yang Y, Teo C, Daumé III H, et al. Corpus-guided sentence generation of natural images[C]//Proceedings of the 2011 conference on empirical methods in natural language processing. 2011: 444-454.
\bibitem{b5} Reiter E. An architecture for data-to-text systems[C]//proceedings of the eleventh European workshop on natural language generation (ENLG 07). 2007: 97-104.
\bibitem{chart2text} Kantharaj S, Leong R T K, Lin X, et al. Chart-to-text: A large-scale benchmark for chart summarization[J]. arXiv preprint arXiv:2203.06486, 2022. 
\bibitem{chartsumm} Rahman R, Hasan R, Farhad A A, et al. Chartsumm: A comprehensive benchmark for automatic chart summarization of long and short summaries[J]. arXiv preprint arXiv:2304.13620, 2023.
\bibitem{b8} Pasupat P, Liang P. Compositional semantic parsing on semi-structured tables[J]. arXiv preprint arXiv:1508.00305, 2015. 
\bibitem{tinychart} Zhang L, Hu A, Xu H, et al. Tinychart: Efficient chart understanding with visual token merging and program-of-thoughts learning[J]. arXiv preprint arXiv:2404.16635, 2024. 
\bibitem{chartqa} Masry A, Long D X, Tan J Q, et al. Chartqa: A benchmark for question answering about charts with visual and logical reasoning[J]. arXiv preprint arXiv:2203.10244, 2022. 
\bibitem{chartstamp} Fu J, Zhu B B, Zhang H, et al. Chartstamp: Robust chart embedding for real-world applications[C]//Proceedings of the 30th ACM International Conference on Multimedia. 2022: 2786-2795. 
\bibitem{deplot} Liu F, Eisenschlos J M, Piccinno F, et al. Deplot: One-shot visual language reasoning by plot-to-table translation[J]. arXiv preprint arXiv:2212.10505, 2022. 
\bibitem{plotqa} Methani N, Ganguly P, Khapra M M, et al. Plotqa: Reasoning over scientific plots[C]//Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision. 2020: 1527-1536. 
\bibitem{textqa} Singh A, Natarajan V, Shah M, et al. Towards vqa models that can read[C]//Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. 2019: 8317-8326. 
\bibitem{b16} Bernardi R, Cakici R, Elliott D, et al. Automatic description generation from images: A survey of models, datasets, and evaluation measures[J]. Journal of Artificial Intelligence Research, 2016, 55: 409-442. 
\bibitem{b17} Hossain M D Z, Sohel F, Shiratuddin M F, et al. A comprehensive survey of deep learning for image captioning[J]. ACM Computing Surveys (CsUR), 2019, 51(6): 1-36. 
\bibitem{b18} Farahani A M, Adibi P, Ehsani M S, et al. Automatic chart understanding: a review[J]. IEEE Access, 2023, 11: 76202-76221. 
\bibitem{GPT4} Achiam J, Adler S, Agarwal S, et al. Gpt-4 technical report[J]. arXiv preprint arXiv:2303.08774, 2023. 
\bibitem{blip2} Li J, Li D, Savarese S, et al. Blip-2: Bootstrapping language-image pre-training with frozen image encoders and large language models[C]//International conference on machine learning. PMLR, 2023: 19730-19742. 
\bibitem{clip} Radford A, Kim J W, Hallacy C, et al. Learning transferable visual models from natural language supervision[C]//International conference on machine learning. PMLR, 2021: 8748-8763. 
\bibitem{blip} Li J, Li D, Xiong C, et al. Blip: Bootstrapping language-image pre-training for unified vision-language understanding and generation[C]//International conference on machine learning. PMLR, 2022: 12888-12900. 
\bibitem{chartllama} Han Y, Zhang C, Chen X, et al. Chartllama: A multimodal llm for chart understanding and generation[J]. arXiv preprint arXiv:2311.16483, 2023. 
\bibitem{matcha} Liu F, Piccinno F, Krichene S, et al. Matcha: Enhancing visual language pretraining with math reasoning and chart derendering[J]. arXiv preprint arXiv:2212.09662, 2022. 
\bibitem{unichart} Masry A, Kavehzadeh P, Do X L, et al. Unichart: A universal vision-language pretrained model for chart comprehension and reasoning[J]. arXiv preprint arXiv:2305.14761, 2023. 
\bibitem{chartinstruct} Masry A, Shahmohammadi M, Parvez M R, et al. ChartInstruct: Instruction Tuning for Chart Comprehension and Reasoning[J]. arXiv preprint arXiv:2403.09028, 2024. 
\bibitem{chartassisstant} Meng F, Shao W, Lu Q, et al. Chartassisstant: A universal chart multimodal language model via chart-to-table pre-training and multitask instruction tuning[J]. arXiv preprint arXiv:2401.02384, 2024. 
\bibitem{qwen2vl} Wang P, Bai S, Tan S, et al. Qwen2-vl: Enhancing vision-language model's perception of the world at any resolution[J]. arXiv preprint arXiv:2409.12191, 2024. 
\bibitem{opencqa} Kantharaj S, Do X L, Leong R T K, et al. Opencqa: Open-ended question answering with charts[J]. arXiv preprint arXiv:2210.06628, 2022. 
\bibitem{monkey} Li Z, Yang B, Liu Q, et al. Monkey: Image resolution and text label are important things for large multi-modal models[C]//Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2024: 26763-26773. 
\bibitem{textmonkey} Liu Y, Yang B, Liu Q, et al. Textmonkey: An ocr-free large multimodal model for understanding document[J]. arXiv preprint arXiv:2403.04473, 2024. 
\bibitem{tinymonkey} Huang M, Liu Y, Liang D, et al. Mini-monkey: Multi-scale adaptive cropping for multimodal large language models[J]. CoRR, 2024. 
\bibitem{llama3} Dubey A, Jauhri A, Pandey A, et al. The llama 3 herd of models[J]. arXiv preprint arXiv:2407.21783, 2024. 
\bibitem{qwen2} Yang A, Yang B, Hui B, et al. Qwen2 technical report[J]. arXiv preprint arXiv:2407.10671, 2024. 
\bibitem{internlm} Team I L M. Internlm: A multilingual language model with progressively enhanced capabilities[J]. 2023-01-06)[2023-09-27]. https://github. com/InternLM/InternLM, 2023. 
\bibitem{llama} Touvron H, Lavril T, Izacard G, et al. Llama: Open and efficient foundation language models[J]. arXiv preprint arXiv:2302.13971, 2023. 
\bibitem{qwen} Bai J, Bai S, Chu Y, et al. Qwen technical report[J]. arXiv preprint arXiv:2309.16609, 2023. 
\bibitem{attention} Vaswani A. Attention is all you need[J]. Advances in Neural Information Processing Systems, 2017. 
\bibitem{b39} Raffel C, Shazeer N, Roberts A, et al. Exploring the limits of transfer learning with a unified text-to-text transformer[J]. Journal of machine learning research, 2020, 21(140): 1-67. 
\bibitem{gopher} Rae J W, Borgeaud S, Cai T, et al. Scaling language models: Methods, analysis \& insights from training gopher[J]. arXiv preprint arXiv:2112.11446, 2021. 
\bibitem{rope} Su J, Ahmed M, Lu Y, et al. Roformer: Enhanced transformer with rotary position embedding[J]. Neurocomputing, 2024, 568: 127063. 
\bibitem{nvlm} Dai W, Lee N, Wang B, et al. Nvlm: Open frontier-class multimodal llms[J]. arXiv preprint arXiv:2409.11402, 2024. 
\bibitem{llava} Liu H, Li C, Wu Q, et al. Visual instruction tuning[J]. Advances in neural information processing systems, 2024, 36. 
\bibitem{b44} Liu H, Li C, Li Y, et al. Improved baselines with visual instruction tuning[C]//Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2024: 26296-26306. 
\bibitem{internvl} Chen Z, Wu J, Wang W, et al. Internvl: Scaling up vision foundation models and aligning for generic visual-linguistic tasks[C]//Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2024: 24185-24198. 
\bibitem{mm1} McKinzie B, Gan Z, Fauconnier J P, et al. MM1: methods, analysis and insights from multimodal LLM pre-training[C]//European Conference on Computer Vision. Springer, Cham, 2025: 304-323. 
\bibitem{blip3} Xue L, Shu M, Awadalla A, et al. xgen-mm (blip-3): A family of open large multimodal models[J]. arXiv preprint arXiv:2408.08872, 2024. 
\bibitem{llavaOV} Li B, Zhang Y, Guo D, et al. Llava-onevision: Easy visual task transfer[J]. arXiv preprint arXiv:2408.03326, 2024. 
\bibitem{flamingo} Alayrac J B, Donahue J, Luc P, et al. Flamingo: a visual language model for few-shot learning[J]. Advances in neural information processing systems, 2022, 35: 23716-23736. 
\bibitem{b50} Zeng Y, Zhang H, Zheng J, et al. What Matters in Training a GPT4-Style Language Model with Multimodal Inputs?[C]//Proceedings of the 2024 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies (Volume 1: Long Papers). 2024: 7930-7957. 
\bibitem{llama_adapter} Zhang R, Han J, Liu C, et al. Llama-adapter: Efficient fine-tuning of language models with zero-init attention[J]. arXiv preprint arXiv:2303.16199, 2023. 
\bibitem{video_llama} Zhang H, Li X, Bing L. Video-llama: An instruction-tuned audio-visual language model for video understanding[J]. arXiv preprint arXiv:2306.02858, 2023. 
\bibitem{qwenvl} Bai J, Bai S, Yang S, et al. Qwen-vl: A frontier large vision-language model with versatile abilities[J]. arXiv preprint arXiv:2308.12966, 2023. 
\bibitem{bert} Devlin, J., Chang, M.-W., Lee, K., and Toutanova, K., BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding, arXiv preprint arXiv:1810.04805, 2018. 
\bibitem{vistext} Tang B J, Boggust A, Satyanarayan A. Vistext: A benchmark for semantically rich chart captioning[J]. arXiv preprint arXiv:2307.05356, 2023. 
\bibitem{pix2struct} Lee K, Joshi M, Turc I R, et al. Pix2struct: Screenshot parsing as pretraining for visual language understanding[C]//International Conference on Machine Learning. PMLR, 2023: 18893-18912. 
\end{thebibliography}
